Unified Pre-training for Program Understanding and Generation

Code summarization and generation empower conversion between programming language (PL) and natural language (NL), while code translation avails the migration of legacy code from one PL to another. This paper introduces PLBART, a sequence-to-sequence model capable of performing a broad spectrum of program and language understanding and generation tasks. PLBART is pre-trained on an extensive collection of Java and Python functions and associated NL text via denoising autoencoding. Experiments on code summarization in the English language, code generation, and code translation in seven programming languages show that PLBART outperforms or rivals state-of-the-art models. Moreover, experiments on discriminative tasks, e.g., program repair, clone detection, and vulnerable code detection, demonstrate PLBART's effectiveness in program understanding. Furthermore, analysis reveals that PLBART learns program syntax, style (e.g., identifier naming convention), logical flow (e.g., if block inside an else block is equivalent to else if block) that are crucial to program semantics and thus excels even with limited annotations.

==> [NAACL 2021] PLBART_camera_ready/images/code_translation.tex <==
\begin{figure*}[!htb]
% \centering
\rule{\textwidth}{0.6pt}
% \vspace{-1mm}
{{Example 1 : \ding{52}}} \\
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Input Code : C\#}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomCS}
\begin{lstlisting}
public int GetCells(){
	int size = 0;
	foreach (char c in cells.Keys){
		Cell e = At(c);
		if (e.cmd >= 0 || e.@ref >= 0){
			size++;
		}
	}
	return size;
}
\end{lstlisting}
\end{tabular}
\end{subfigure}%
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Generated Code : Java}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
public int getCells() {
	Iterator<Character> i = 
	    cells.keySet().iterator();
	int size = 0;
	for (; i.hasNext();) {
		Character c = i.next();
		Cell e = at(c);
		if (e.cmd >= 0 || e.ref >= 0){
			size++;
		}
	}
	return size;
}
\end{lstlisting}
\end{tabular}
\end{subfigure}
\rule{\linewidth}{0.6pt}

{{Example 2 : \ding{52}}} \\
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Input Code : C\#}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomCS}
\begin{lstlisting}
public override Cell Merge(
    Cell m, Cell e){
	if (m.cmd == e.cmd && m.@ref == 
	  e.@ref && m.skip == e.skip) {
		Cell c = new Cell(m);
		c.cnt += e.cnt;
		return c;
	} 
	else {
		return null;
	}
}
\end{lstlisting}
\end{tabular}
\end{subfigure}%
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=~,style=CustomJava}
\caption{\underline{Generated Code : Java}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
public Cell merge(Cell m, Cell e) {
	if (m.cmd == e.cmd && 
		m.ref == e.ref && 
		m.skip == e.skip) {
		Cell c = new Cell(m);
		c.cnt += e.cnt;
		return c;
	} 
	else {
		return null;
	}
}
\end{lstlisting}
\end{tabular}
\end{subfigure}

\rule{\linewidth}{0.6pt}

{{Example 3 : \ding{52}}}\\
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Input Code : Java}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
@Override public List<E> subList(
    int start, int end) {
	synchronized (mutex) {
		return new 
		    SynchronizedRandomAccessList
		    <E>(
			list.subList(start, end), 
			mutex);
	}
}
\end{lstlisting}
\end{tabular}
\end{subfigure}%
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Generated Code : C\#}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomCS}
\begin{lstlisting}
public override java.util.List<E> 
    SubList(int start, int end){
	lock (mutex){
		return new java.util.Collections.
		    SynchronizedRandomAccessList<E>(
			list.subList(start, end), 
			mutex
		);
	}
}
\end{lstlisting}
\end{tabular}
\end{subfigure}

\rule{\linewidth}{0.6pt}

{{Example 4 : \ding{52}}}\\
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Input Code : Java}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
public 
    PersianNormalizationFilterFactory(
		Map<String,String> args) {
	super(args);
	if (!args.isEmpty()) {
		throw 
		    new IllegalArgumentException(
			    "Unknown parameters: " 
			    + args);
	}
}
\end{lstlisting}
\end{tabular}
\end{subfigure}%
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Generated Code : C\#}}
% \vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomCS}
\begin{lstlisting}
public 
    PersianNormalizationFilterFactory(
	IDictionary<string, string> args) 
	        : base(args){
	if (args.Count > 0){
		throw new System.ArgumentException(
			"Unknown parameters: " 
			+ args
		);
	}
}
\end{lstlisting}
\end{tabular}
\end{subfigure}
\rule{\linewidth}{0.6pt}
\caption{
Qualitative examples of source code translation between Java and C\# using PLBART.
}
\label{cs_java_example}
% \vspace{-2mm}
\end{figure*}

==> [NAACL 2021] PLBART_camera_ready/images/qual_example_concode.tex <==
\begin{figure}[t]
% \centering
\rule{\linewidth}{0.6pt}
% \vspace{-1mm}
{{\bf Input text:} returns the count to which the specified key is mapped in this frequency counter , or 0 if the map contains no mapping for this key .}
\\ [8pt]
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Reference Code}}
\vspace{-1mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
Integer function (T arg0) { 
	Integer loc0 = counter.get(arg0); 
	if (loc0 == null) { 
		return 0 ;
	} 
	return loc0; 
}
\end{lstlisting}
\end{tabular}
\label{tab:ref_code_concode}
\end{subfigure}%
\\ \\
% \vspace{2mm}
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Generated Code}}
\vspace{-1mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
int function (T arg0) { 
	Integer loc0 = counter.get(arg0); 
	if (loc0 == null) { 
		return 0 ;
	} 
	else { 
		return loc0;
	} 
}
\end{lstlisting}
\end{tabular}
% \vspace{1mm}
\label{tab:gen_code_concode}
\end{subfigure}
% \vspace{1mm}
\rule{\linewidth}{0.6pt}
\caption{
An example of generated code by PLBART that is syntactically and semantically valid, but does not match the reference.
}
\label{concode_example}
\vspace{-2mm}
\end{figure}

==> [NAACL 2021] PLBART_camera_ready/images/qual_example_concode_2.tex <==
\begin{figure}[t]
% \centering
\rule{\linewidth}{0.6pt}\vspace{-1mm}
{{\bf Input text:} returns the count to which the specified key is mapped in this frequency counter , or 0 if the map contains no mapping for this key .}
\\ [6pt]
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Reference Code}}
\vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
Integer function (T arg0) { 
	Integer loc0 = counter.get(arg0); 
	if (loc0 == null) { 
		return 0 ;
	} 
	return loc0; 
}
\end{lstlisting}
\end{tabular}
\label{tab:ref_code_concode}
\end{subfigure}%
\\ \\
% \vspace{2mm}
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Generated Code}}
\vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
int function (T arg0) { 
	Integer loc0 = counter.get(arg0); 
	if (loc0 == null) { 
		return 0 ;
	} 
	else { 
		return loc0;
	} 
}
\end{lstlisting}
\end{tabular}
% \vspace{1mm}
\label{tab:gen_code_concode}
\end{subfigure}
% \vspace{1mm}
\rule{\linewidth}{0.6pt}
\caption{
An example of generated code by PLBART that is syntactically and semantically valid, but does not match the reference.
}
\label{concode_example}
% \vspace{-2mm}
\end{figure}

==> [NAACL 2021] PLBART_camera_ready/images/qual_example_cs_to_java.tex <==
\begin{figure}[t]
% \centering
\rule{\linewidth}{0.6pt}
% {{Example  : \xmark}}\\
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Reference Code : C\#}}
\vspace{-1mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomCS}
\begin{lstlisting}
public bool find(int start_1){
	findPos = start_1;
	...
	else{
		if (findPos >= _regionEnd){
			matchFound = false;
			return false;
		}
	}
	...
}
\end{lstlisting}
\end{tabular}
\label{tab:Example_1_Cs_to_java}
\end{subfigure}%
\\ \\
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Generated Code : C\#}}
\vspace{-1mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomCS}
\begin{lstlisting}
public bool find(int start){
	findPos = start;
	...
	else if (findPos >= _regionEnd){
		matchFound = false;
		return false;
	}
	...
}
\end{lstlisting}
\end{tabular}
\end{subfigure}
\rule{\linewidth}{0.6pt}
\caption{
Example C\# code generated by \tool that does not exactly match the reference code.
}
\label{code_trans_example}
\vspace{-2mm}
\end{figure}

==> [NAACL 2021] PLBART_camera_ready/latex/conclusion.tex <==
\section{Conclusion}
This paper presents PLBART, a sizeable pre-trained sequence-to-sequence model that can perform program and language understanding and generation tasks. PLBART achieves state-of-the-art performance on various downstream software engineering tasks, including code summarization, code generation, and code translation. Furthermore, experiments on discriminative tasks establish PLBART's effectiveness on program understanding. We also show that PLBART learns crucial program characteristics due to pre-training, such as syntax, identifier naming conventions, data flow. In the future, we want to explore ways to fine-tune PLBART on all the downstream tasks jointly.


==> [NAACL 2021] PLBART_camera_ready/latex/experiment.tex <==
\section{Results \& Analysis}
% In this section, we present and analyze the evaluation results based on the tasks we defined in pre~\cref{sec:exp_setup}.
We aim to address the following questions.
\begin{compactenum}
    \item Does PLBART learn strong program and language representations from unlabeled data?
    \item Does PLBART learn program characteristics, \eg syntax, style, and logical data flow?
    \item How does PLBART perform in an unseen language with limited annotations?
\end{compactenum}


\input{table/text_to_code}
\input{images/qual_example_concode}
\input{table/code_to_code}



\subsection{Code Summarization}

\Cref{table:code_to_text} shows the result of code summarization.
PLBART outperforms the baseline methods in five out of the six programming languages with an overall average improvement of 0.49 BLEU-4 over CodeBERT.
The highest improvement ($\sim$16\%) is in the Ruby language, which has the smallest amount of training examples.
Unlike CodeBERT, PLBART is not pretrained on the Ruby language; however, the significant performance improvement indicates that PLBART learns better generic program semantics.
% \notekw{in BLEU-4? specify the metric as ``points'' is kind of vague} 
% PLBART outperforms CodeBERT by 16\%, 4.4\%, 4.6\%, 4.5\%, and 1.3\% in Ruby, Javascript, Go, Python, and Java languages, respectively.
% In PHP, PLBART performs poorly compared to CodeBERT and RoBERTa. 
% Note that, CodeBERT is pretrained and finetuned on all six languages using CodeSearchNet, while PLBART is only pretrained on Java and Python using a different data source. 
% Therefore, PLBART's superior or comparable performance on other languages indicate that PLBART learns to understand programs beyond the programming language syntax. 
% It is also worth noting that PLBART is not pretrained on four of the 
% Therefore, PLBART's superior or comparable performance in other languages indicates that it learns better program semantics irrespective of the language.
% This claim is also corroborated while comparing with Transformer baseline. 
% PLBART's better performance over transformer demonstrates the effectiveness of the pretraining step.
In contrast, PLBART performs poorly in the PHP language. The potential reason is syntax mismatch between the pre-trained languages and PHP. 
% As a result, PLBART has a smaller gain over Transformer ($\sim$1.5 points). 
Surprisingly, RoBERTa performs better than PLBART on the PHP language. 
We suspect that since RoBERTa is pre-trained on natural language only, it does not suffer from the syntax mismatch issue.
Overall in comparison to the Transformer baseline, PLBART improves with an average of 2.76 BLEU-4, and we credit this improvement to the pre-training step.
% and adds a $\sim$2.0 points gain over Transformer. 
% CodeBERT's performance is understandable as one of its pre-training languages is PHP. 
% Moreover, compared 


% We suspect that PLBART’s understanding of programming language learned during pre-training conflicts when it observes PHP language. 



\subsection{Code Generation}

\Cref{table:concode} shows the evaluation result on code generation from NL description.
PLBART outperforms all the baselines in terms of BLEU and CodeBLEU. 
While CodeGPT-adapted~\cite{CodeXGLUE} achieves the best Exact Match (EM) score, PLBART outperforms CodeGPT-adapted by a large margin in terms of CodeBLEU. 
This result implies that PLBART generates \emph{significantly more} syntactically and logically correct code than all the baselines.


~\Cref{concode_example} shows an example of code generated by PLBART.
% which does not exactly match the reference. 
The difference between the reference code and the generated code is in line 6 onward. In the reference code, {\tt loc0} is returned, however same {\tt loc0} is returned in an {\tt else} block in the generated code. If we look closely, in the reference code, line 6 will be executed only if the condition in line 3 (\ie {\tt loc0 == null}) is {\tt false}. In the generated code, {\tt loc0} will be returned only if the condition in line 3 is {\tt false}, making the generated code semantically equivalent to the reference code. 
% While the reference code clears the {\tt buffer} by setting the {\tt bufferSize} to 0, PLBART's generated code does it by setting {\tt buffer} to {\tt null}. 
% As we can see the reference code clears the {\tt buffer} by setting the {\tt bufferSize} to 0, PLBART does the same by setting {\tt buffer} to {\tt null}.
% Since, {\tt buffer} is a byte array (mentioned in the input text), setting it to {\tt null} does not violate program semantics. 
% To understand PLBART's resilience to learn from small data, The Concode dataset contains 100K training examples. 


To study whether PLBART learns code syntax and logical flow during pre-training or fine-tuning, we perform an ablation study where we use subset of the training examples (10K, 20K, and 50K) to fintune PLBART in this task.
% More specifically, we finetune PLBART with 10K (PLBART$_{10K}$), 20K (PLBART$_{10K}$), and 50K (PLBART$_{10K}$) training examples. 
As \cref{table:concode} shows, with only 10K examples, PLBART outperforms all baselines in terms of CodeBLUE. 
This ablation shows that PLBART learns program syntax and data flow during pre-training, resulting in effective performance on downstream tasks even when finetuned on small number of examples.

As shown in prior works~\cite{yin-neubig-2017-syntactic, chakraborty2020codit}, generating syntactically and logically correct code has been a big challenge in program generation.
We conjecture that PLBART's large-scale denoising sequence-to-sequence pre-training helps understand program syntax and logical flow; therefore enables PLBART to generate syntactically and logically valid code.



\subsection{Code Translation}

% \Cref{table:code_translation} shows PLBART's performance in code translation from one programming language to another. 
% We present the evaluation results in \Cref{table:code_translation}.
\Cref{table:code_translation} presents the evaluation results on code translation.
PLBART outperforms all the baselines \wrt EM, BLEU, and CodeBLEU. 
PLBART improves over CodeBERT by 9.5\% and 10.5\% when translating from Java to C\# and C\# to Java, respectively.
Although PLBART is not pretrained on C\# language, there is a significant syntactic and semantic similarity between Java and C\#. Thus PLBART understands C\# language syntax and semantics. 
However, such similarities are non-trivial, making the Naive copy and PBSMT perform very poorly in both the translation tasks.
% When translating from Java code to C\#, PLBART can generate 9.5\% more code than CodeBERT baseline that exactly matches the reference. 
% PLBART can also generate 10.5\% more exact matches with reference than CodeBERT when translating from C\# to Java. 
% in both the translation tasks. 



\input{images/qual_example_cs_to_java}


\Cref{code_trans_example} shows an example where PLBART's generated C\# code does not exactly match the reference; however, they are semantically equivalent. 
% However, the generated is semantically equivalent to the reference code. 
% In the reference code, single {\tt if} block (line 5-8) inside the {\tt else} block (line 4-9) is equivalent with the generated code's {\tt else if} block (line 4-7), given that everything inside is generated as expected. 
In the reference, the {\tt else} block (line 4-9) is equivalent to the {\tt else if} block (line 4-7) in the generated code.
% This shows the syntactic understanding of PLBART. 
In addition, {\tt start} is generated as function parameter and used in the function body, equivalent to {\tt start\_1} in the reference code. 
This further corroborates the syntactic understanding of PLBART and its ability to reason about the data flow in source code. 
We present more qualitative examples in Appendix.
% This further corroborates PLBART's ability to reason about the data flow in source code.


In the program repair task, both the input and the output are in the same language.
While the input is a buggy code, the output should be the target bug-free code.
Thus in this task, the exact match is the critical metric.
Nevertheless, as shown in~\cref{table:bug_fix}, PLBART can generate 17.13\%, and 74.03\% more correct bug fixes than CodeBERT in Java$_{small}$ and Java$_{medium}$ datasets, respectively. 
On the other hand, PLBART performs comparably to GraphCodeBERT that uses structure-aware pre-training to learn program syntax and semantics.
% , translation is a bit difficult, since there is a semantic difference between the input and output code. 
% Because, unless a buggy code is transformed in a certain and desired way, it is not considered fixed, no matter how similar it is to the original fix. 

% GraphCodeBERT~\cite{guo2020graphcodebert} reported 17.30\% EM in Java$_{small}$, and 9.10\% in Java$_{medium}$. 
% While their results are comparable with PLBART's result, their model is much more sophisticated than PLBART, since they used explicit syntax and semantics encoded into the model. 





\subsection{Classification}


In both clone detection and the vulnerability detection tasks, PLBART outperforms CodeBERT. We present the results in Table \ref{table:classification}.
% For Vulnerability detection task, the input code are written in C, which is not used in PLBART's pretraining. 
% A transformer based classification model (\emph{without} the PLBART pretraining) achieve accuracy of 61.64\%. 
% We pretrain a Transformer encoder for vulnerability detection and it achieves 61.64\% accuracy. 
In the vulnerability detection task, code semantics is the most critical feature \cite{zhou2019devign, chakraborty2020deep}. 
Since PLBART is not pretrained on C/C++ language, its improved performance compared to the Transformer baseline is the testament that PLBART can identify semantics beyond the language syntax's specifics.
Moreover, PLBART's improved performances over CodeBERT and GraphCodeBERT confirms its effectiveness in program understanding in addition to its generation ability.
% Moreover, CodeBERT and GraphCodeBERT are BERT-style model and more suitable for program understanding (\ie classification) tasks, however, PLBART's improved performances over them shows its ability in generic understanding of program semantics in addition to its generation ability.



\input{table/repair}
\input{table/vulnerability}


We acknowledge that neither PLBART nor CodeBERT is state-of-the-art in vulnerability detection, as graph-based models perform best in this task. 
In this evaluation, our goal is to study how well PLBART understands program semantics in an unseen language for a different type of task (other than the generation, \ie classification).
% explicitly encoding different semantic dependencies performs best for this task. 
% In this evaluation, it is not our goal to evaluate PLBART's (or any other models') performance in vulnerability detection, rather we want to study how well PLBART understands program in an unseen language for a different type of task (\ie classification).
% As for the Clone detection task, PLBART also outperforms CodeBERT. 




==> [NAACL 2021] PLBART_camera_ready/latex/introduction.tex <==
\section{Introduction}

%Engineers and developers use a programming language (PL) to write software programs and natural language (NL) to communicate them.
%The use of natural language includes writing documentation, commit messages, bug reports, seeking help in different forums (\eg Stack Overflow), etc.
% Engineers and developers write software programs in a programming language (PL) like Java, Python, etc., and often use natural language (NL) to communicate them. For example, they use natural language to write documentation, commit messages, bug reports, seek help in different forums (\eg Stack Overflow), etc.
% The use of NL in software development are often colloquially different from written and spoken language. 
% For instance, when software engineers use \emph{Code Smell\footnote{https://en.wikipedia.org/wiki/Code\_smell}}, it means potential problem in code (something other than \emph{Smell} in regular English language). 
% Automation of software development and maintenance requires the understanding of PL and NL.\footnote{In this paper, we consider natural language in the context of software development and maintenance.}
% Software engineering applications, such as source code summarization, generation and translation solely rely on program and language understanding.
% We collectively refer them as PLUG (stands for, Program and Language Understanding and Generation) applications or tasks.

Engineers and developers write software programs in a programming language (PL) like Java, Python, etc., and often use natural language (NL) to communicate with each other.
% For example, English is commonly 
Use of NL in software engineering ranges from writing documentation, commit messages, bug reports to seeking help in different forums (\eg Stack Overflow), etc. 
Automating different software engineering applications, such as source code summarization, generation, and translation, heavily rely on the understanding of PL and NL---we collectively refer them as PLUG (stands for, Program and Language Understanding and Generation) applications or tasks.
% \footnote{In this paper, we consider natural language in the context of software development and maintenance.}
% However,  PL and the use of NL in software development are quite different than colloquially written and spoken language. While PL can have an arbitrary vocabulary, unambiguous semantics, etc., the NL in software development often contains domain-specific jargon. For instance, when software engineers use \emph{Code Smell\footnote{https://en.wikipedia.org/wiki/Code\_smell}}, it means a potential problem in code (something other than \emph{Smell} in regular English language).
Note that the use of NL in software development is quite different than colloquially written and spoken language. 
% While PL can have an arbitrary vocabulary, unambiguous semantics, etc., the NL in software development often contains domain-specific jargon. 
% While PL can have an arbitrary vocabulary, unambiguous semantics, etc., the NL in software development often contains domain-specific jargon. 
% For instance, when software engineers use \emph{Code Smell\footnote{https://en.wikipedia.org/wiki/Code\_smell}}, it means a potential problem in code (something other than \emph{Smell} in regular English language).
For example, NL in software development often contains domain-specific jargon, \eg when software engineers use \emph{Code Smell\footnote{https://en.wikipedia.org/wiki/Code\_smell}}, it means a potential problem in code (something other than \emph{Smell} in regular English language).


\input{images/example}

In this work, our goal is to develop a general-purpose model that can be used in various PLUG applications.
Recent advancements in deep learning and the availability of large-scale PL and developers' NL data ushered in the automation of PLUG applications. 
% However, as opposed to  mainstream natural language applications,
% directly applying existing NLP models is challenging as
% However, as opposed to  mainstream natural language applications,
One important aspect of PLUG applications is that they demand a profound understanding of program syntax and semantics and mutual dependencies between PL and NL. 
% {\color{red} Such understandings are difficult because of the structured }
For example,~\Cref{main_example_2} shows two implementations of the same algorithm (sorting) in two PL and corresponding NL summary.
% An automatic tool that translates the Python code to Java must understand that function {\tt sorted} in {Python} acts similar to {\tt Arrays.sort} in {Java} and the {\tt lambda} operation in {Python} is equivalent to instantiating a {\tt Comparator} object in {Java}. 
An automatic translation tool must understand that function {\tt sorted} in {Python} acts similar to {\tt Arrays.sort} in {Java} and the {\tt lambda} operation in {Python} is equivalent to instantiating a {\tt Comparator} object in {Java}.
Similarly, a tool that summarizes either of these code must understand that {\tt x[0]} in {Python} or {\tt Tuple.get(0)} in {Java} refers to the first element in the tuple list.
% Similarly, a tool that summarizes either of these code must understand that {\tt x[0]} in {Python} or {\tt Tuple.get(0)} in {Java} refers to the first element in the tuple list.

% and often requires to migrate them into another language.
% and associated natural language to communicate about the program.
% Along with writing code using different Programming Languages (PL), engineers write documentation, commit message, bug report using Natural Language (NL). 
% Developers also extensively use different forums (\eg Stack Overflow) to get help from others. 
% Thus, an automated tool aiming at helping them do different programming related task, must understand syntax and semantics of the source code (written in PL) and how those are related to text (written in NL). 
% It is worth noting that use of NL in programming tasks are often colloquially different from written and spoken language. 
% For instance, when software engineers use \emph{Code Smell\footnote{https://en.wikipedia.org/wiki/Code\_smell}}, it means something other than \emph{Smell} in ordinary English. 

% In this work, our goal is to develop a general-purpose technique that can be applied for a wide variety of PLUG tasks. 
% % Learning proper representation learning model that understands program and language syntax and semantics and capable of performing PLUG tasks.
% Recent advancement in deep learning and availability of large scale PL and developers' NL data ushered the opportunity of automating PLUG tasks. 
% However, most of these data are unlabeled and cannot be utilized across tasks, \eg program generation and translation.
% % For example, parallel Java and NL corpora are available, but Java to C/C++ or Python annotations are unavailable.
% Therefore, learning one model to perform a variety of tasks is challenging. 


% In recent years, we have seen a colossal effort to pre-train encoders on massive amount of unlabeled data (\eg text, images, videos) \cite{devlin2018bert, liu2019roberta, NIPS2019_8928, conneau-etal-2020-unsupervised, li-etal-2020-bert-vision, sun2019videobert}.
% % that are trained on bimodal data (e.g., language-image or language-video).
% % These encoders are pre-trained in a self-supervised fashion, primarily using masked language modeling (MLM) \cite{devlin2018bert}.
% This inspired researchers to develop general purpose representation encoders for PL and NL, such as CodeBERT \cite{feng2020codebert} and GraphCodeBERT \cite{guo2020graphcodebert}.
% These PL-NL encoders are pretrained on a \emph{small-scale} bimodal data (code-text pairs) and have been found useful for many PLUG applications, including code search, code completion, program repair, clone detection, and more.
% However, they have limited use in autoregressive tasks, such as code summarization, generation, and translation.
% , where an input text is randomly masked and the encoders are trained to predict the masked tokens based on available context.
% The encoders are then fine-tuned on particular types of downstream tasks (e.g., classification, token prediction, etc.). 
% \notebr{why? Can you give any intuition how you can address them?}.

%In this work, our goal is to develop a general-purpose model that can be used for a wide variety of PLUG tasks. 
%Recent advancement in deep learning and availability of large scale PL and developers' NL data ushered the opportunity of automating PLUG tasks. 
% msg from KW
% This part is weird. Even if you learn a good representation model, you still cannot solve this problem and learn a unified model right? Also, the first sentence reads like the unlabeled data cannot be used across different task, but that is exactly what you proposed to do to leverage unlabeled data to improve over multiple tasks. I think what you want to say the annotation is expensive however, different problem and different languages shared the common ground. Therefore if we can learn a good representation model then we can use less label data to achieve the goal.
Most of the available data in PL and NL are unlabeled and cannot be trivially used to acquire PLUG task-specific supervision.
However, PLUG tasks have a common prerequisite \textemdash~understanding PL and NL syntax and semantics.
% across different tasks.
% for task specific supervision. 
% However, one important aspect about PLUG tasks is that they share common goal of understanding and generating PL and NL irrespective of the task.
Leveraging unlabelled data to pretrain a model to learn PL and NL representation can be transferred across PLUG tasks.
This approach reduces the requirement of having large-scale annotations for task-specific fine-tuning.
% Such a pre-trained model can later be fine-tuned with small set of task specific supervision.
% ~\notewa{What do you mean by task specific supervision?}
% cannot be utilized across tasks, \eg program generation and translation.
% Therefore, learning a unified model to perform a variety of tasks is challenging. 
% To solve this problem, we aim to design a representation learning model that understands program and language syntax and semantics.
In recent years we have seen a colossal effort to pretrain models on a massive amount of unlabeled data (\eg text, images, videos) \cite{devlin-etal-2019-bert, liu2019roberta, NIPS2019_8928, conneau-etal-2020-unsupervised, li2019visualbert, sun2019videobert}
to transfer representation encoders across a wide variety of applications.
% Such approach takes inspiration from the colossal efforts to pretrain models on a massive amount of unlabeled data (\eg text, images, videos) \cite{devlin2018bert, liu2019roberta, NIPS2019_8928, conneau-etal-2020-unsupervised, li2019visualbert, sun2019videobert}.
There are a few research effort in learning general purpose PL-NL representation encoders, such as CodeBERT~\cite{feng2020codebert} and GraphCodeBERT~\cite{guo2020graphcodebert} that are pretrained on a \emph{small-scale} bimodal data (code-text pairs). 
Such models have been found effective for PLUG tasks, including code search, code completion, etc. 

Language generation tasks such as code summarization is modeled as sequence-to-sequence learning, where an encoder learns to encode the input code and a decoder generates the target summary. Despite the effectiveness of existing methods, they do not have a pretrained decoder for language generation. Therefore, they still require a large amount of parallel data to train the decoder. To overcome this limitation, \citet{lewis-etal-2020-bart} proposed denoising sequence-to-sequence pre-training where a Transformer \cite{vaswani2017attention} learns to reconstruct an original text that is corrupted using an arbitrary noise function. Very recently, \citet{lachaux2020unsupervised} studied denoising pre-training using a large-scale source code collection aiming at unsupervised program translation and found the approach useful.
% However, these models have an encoder and are combined with a decoder to perform generative tasks autoregressively via task-specific fine-tuning.
% The autoregressive decoder is trained from scratch which limits their usage in settings where there is a limited annotations available.
% they have limited use in autoregressive tasks, such as code summarization, generation, and translation. 
% "The PLUG tasks such as code summarization can be modeled as a sequence-to-sequence task, where a model learn to encode the code snippet and generate the corresponding text summary. Despite existing methods in PL-NL prepresentatoins, such as CodeBERT, ... GraphCodeBERT, learn a useful representation model for the encoder, they do not have pre-trained model for the decoder. Therefore, they there still need a large amount of pair data to train the decoder.
% To facilitate autoregressive tasks using unlabeled data, denoising sequence-to-sequence pre-training using Transformers \cite{vaswani2017attention} has found success \cite{lewis-etal-2020-bart}.
% In contrast, denoising sequence-to-sequence pre-training using Transformers \cite{vaswani2017attention} leveraging unlabeled data has facilitated many autoregressive NLP applications \cite{lewis-etal-2020-bart}.
% According to the pre-training approach, Transformers learn to reconstruct an original text that is corrupted using an arbitrary noise function.
This raises a natural question, \emph{can we unify pre-training for programming and natural language?}
% We take this as a motivation to pre-train a Transformer model on programming and natural languages jointly.
Presumably, to facilitate such pre-training, we need unlabeled NL text that is relevant to software development.
Note that unlike other bimodal scenarios (\eg vision and language), PL and associated NL text share the same alphabet or uses anchor tokens (\eg ``sort'', ``list'', ``tuple'' as shown in \Cref{main_example_2}) that can help to learn alignment between semantic spaces across languages.
% We hypothesize that since PL and NL uses the same alphabet or anchor tokens (\eg ``sort'', ``list'', ``tuple'' as shown in \Cref{main_example_2}), PLBART learns to align between the embedding spaces across languages.

% msg from kw
% It not clear to the readers what is the key innovation in your model. Do you have a new learning/pre-training objective? -- how you actually address the research question you ask.
We introduce PLBART (Program and Language BART), a bidirectional and autoregressive transformer pre-trained on unlabeled data across PL and NL to learn multilingual representations applicable to a broad spectrum of PLUG applications.
% on Java and Python functions and StackOverflow posts.
% a bidirectional and autoregressive transformer pre-trained via denoising autoencoding on two widely used programming language (PL): Java and Python, and natural language (NL) English.
% PLBART is pretrained on 680M Java and Python functions collected from Github and 47M StackOverflow posts written in NL.
% PLBART uses unlabeled data across PL and NL to learn multilingual representations applicable to a broad spectrum of applications.
We evaluate PLBART on code summarization, generation, translation, program repair, clone detection, and vulnerability detection tasks.
Experiment results show that PLBART outperforms or rivals state-of-the-art methods, \eg CodeBERT and GraphCodeBERT, demonstrating its promise on program understanding and generation.
We perform a thorough analysis to demonstrate that PLBART learns program syntax, logical data flow that is indispensable to program semantics, and excels even when limited annotations are available.
We release our code\footnote{https://github.com/wasiahmad/PLBART} to foster future research.




% {\color{red}
% Our goal in this research is to develop a tool that automate a wide variety of Software Engineering (SE) tasks that requires understanding of PL and NL.
% help engineers across a wide variety of software engineering tasks that deal with PL and NL. 
% We collectively refer such tasks as PLUG (stands for, Program and Language Understanding and Generation).
% family of tasks. 


% To understand characteristics of PLUG tasks even further, let's look at the example shown in~\Cref{main_example_2} showing two different implementation (in {Java}, and {Python}) of the same algorithm and corresponding NL summary.
% While the example is very trivial, a tool that translates legacy Python code to Java must understand that function {\tt sorted} in {Python} acts similar to {\tt Arrays.sort} in {Java} and the {\tt lambda} operation in {Python} should translate to instantiating a {\tt Comparator} object in {Java}. 
% A tool that summarizes either of these code must understand that {\tt x[0]} in {Python} or {\tt Tuple.get(0)} in {Java} translates to the first element in a tuple. 
% Clearly, such tasks demand a profound understanding of program syntax and semantics as well as mutual dependencies between PL and NL. 

% We formulate the problem of solving PLUG tasks as developing a model with deeper understanding of the programs and languages. Such a model should learn the code syntax, learn about the APIs in code, understand the code semantics beyond the PL syntax and generalize across different PLs, learn about the programming style, and  learn about the mutual dependencies between PL and programmers' NL.
% \notesc{}

% \notewa{Our novelty is not in the technical side, rather we develop a model that can perform program understanding and generation task, e.g., vulnerability or clone detection, code summarization and generation.}

% Source code summarization, generation and translation tasks require comprehensive understanding of programming language (PL) and natural language (NL).
% ~\notebr{It is not clear how PL is connected with NL}. 
% \notewa{We focus on natural language that developers use for software development and maintenance, such as commit messages, issues, readme files etc.}
% This paper 
% Figure \ref{main_example} shows an example of parallel expressions across NL and PL.

% Automatic conversion of these expressions from one language to another can greatly help software development and maintenance.
% Automation of these tasks can greatly help software development and maintenance. 
% Due to the advancement of deep learning and large-scale data availability, automating PLUG applications has drawn attention from researchers.
% Consequently, several methods have been developed, however, there was no general-purpose model that can be adapted to many of the PLUG applications until recently.


% Recent advancement in deep learning and availability of large scale PL and developers' NL data ushered the opportunity of automating PLUG tasks. While there are a number of research approaches for individual tasks in PLUG family of task, very few formulate those as generalized PLUG task.
% } 

% In recent years, we have seen a colossal effort to pre-train language encoders on massive amount of unlabeled natural language text in one language or jointly on many languages using Transformer \cite{vaswani2017attention}. Noteworthy language encoders, such as, BERT \cite{devlin2018bert} , RoBERTa \cite{liu2019roberta}, XLM \cite{NIPS2019_8928} and XLM-R \cite{conneau-etal-2020-unsupervised} have revolutionized natural language processing (NLP). The success of the pre-trained encoders in NLP resulted in pre-training multi-modal encoders, such as VisualBERT \cite{li-etal-2020-bert-vision} or VideoBERT \cite{sun2019videobert}.
% % that are trained on bimodal data (e.g., language-image or language-video).
% This inspired researchers to develop CodeBERT \cite{feng2020codebert}, GraphCodeBERT \cite{guo2020graphcodebert}; general purpose representation encoders for PL and NL that are pre-trained on 2.4M code-text pairs from CodeSearchNet \cite{husain2019codesearchnet}.
% These PL-NL encoders have been found useful for many PLUG applications, including code search, code completion, program repair, clone detection, and more.


==> [NAACL 2021] PLBART_camera_ready/latex/method.tex <==
\section{PLBART}
\label{sec:method}
% PLBART uses denoising sequence-to-sequence pre-training \cite{lewis-etal-2020-bart} for programming language (PL) and natural language (NL) generation, translation, and comprehension.
% We detail the pre-training of PLBART in this section.
PLBART uses denoising sequence-to-sequence pre-training to utilize unlabeled data in PL and NL. Such pre-training lets PLBART reason about language syntax and semantics.
At the same time, PLBART learns to generate language coherently.
% Such pre-training lets PLBART reason about the syntax and semantics of the inputs (both PL and NL). 
% At the same time, decoder of the model learns to generate grammatically and logically correct input.

\input{table/pretrain_data}
% \begin{figure*}[t]
% \centering
% \includegraphics[width=1.0\linewidth]{images/pretraining.png}
% \caption{caption. will replace this figure.} 
% \label{fig:method}
% % \vspace{-2mm}
% \end{figure*}

\input{table/example1}


\subsection{Denoising Pre-training}

\paragraph{Data \& pre-processing}
% \noindent\textbf{Data \& pre-processing \hspace{0.5em}}
We pre-train PLBART on a large-collection of Java and Python functions and natural language descriptions from Github and StackOverflow, respectively.
We download all the GitHub repositories associated with Java and Python languages available on Google BigQuery.\footnote{https://console.cloud.google.com/ marketplace/details/github/github-repos}
We extract the Java and Python functions following the pre-processing pipeline from \citet{lachaux2020unsupervised}.
We collect the StackOverflow posts (include both questions and answers, exclude code snippets) by downloading the data dump (date: 7th September 2020) from stackexchange.\footnote{https://archive.org/download/stackexchange}
Statistics of the pre-training dataset are presented in Table \ref{table:pretrain_data}.
We tokenize all the data with a sentencepiece model \cite{kudo-richardson-2018-sentencepiece} learned on 1/5'th of the pre-training data.
We train sentencepiece to learn 50,000 subword tokens.
% We do not perform any additional pre-processing, such as normalizing punctuation/characters.

One key challenge to aggregate data from different modalities is that some modalities may have more data, such as we have 14 times more data in PL than NL. 
Therefore, we mix and up/down sample the data following \citet{NIPS2019_8928} to alleviate the bias towards PL. 
We sample instances for pre-training according to a multinomial distribution with probabilities $(q_1, q_2, \ldots, q_N)$:
\begin{equation*}
    q_i = \frac{1}{p_i} \cdot \frac{p_i^{\alpha}}{\sum_{j=1}^N p_j^{\alpha}}, 
    p_i = \frac{n_i}{\sum_{j=1}^N n_j},
\end{equation*}
where $N$ is the total number of languages and $n_i$ is the total number of instances in language $i$.
We set the smoothing parameter $\alpha$ to 0.3.



\input{table/example2}


\paragraph{Architecture}
% \smallskip
% \noindent\textbf{Architecture \hspace{0.5em}}
PLBART uses the same architecture as BART$_{base}$ \cite{lewis-etal-2020-bart}, it uses the sequence-to-sequence Transformer architecture \cite{vaswani2017attention}, with 6 layers of encoder and 6 layers of decoder with model dimension of 768 and 12 heads ($\sim$140M parameters). 
The only exception is, we include an additional layer-normalization layer on top of both the encoder and decoder following \citet{liu2020multilingual}, which is found to stabilize training with FP16 precision.
% We initialise the parameters from $\mathcal{N} (0, 0.02)$.


\paragraph{Noise function, $f$} 
% \smallskip
% \noindent\textbf{Noise function, $f$ \hspace{0.5em}} 
% \notekw{You need to describe first what is the noise function used in the pre-training. We cannot assume people read the BART paper. I think you need to add a paragraph to summarize this denoising pre-training process in the begining of Sec 2.1}
In denoising autoencoding, a model learns to reconstruct an input text that is corrupted by a noise function.
Reconstruction of the original input requires the model to learn language syntax and semantics.
% Reconstruction of the original input lets the model reason about the language syntax and semantics as well as train the model generate syntactically and semantically correct input.
In this work, we use three noising strategies: token masking, token deletion, and token infilling \cite{lewis-etal-2020-bart}.
According to the first two strategies, random tokens are sampled and replaced with a mask token or deleted from the input sequence.
In token infilling, a number of text spans are sampled and replaced with a \emph{single} mask token.
The span lengths are drawn from a Poisson distribution ($\lambda = 3.5$).
We mask 35\% of the tokens in each instance.


\paragraph{Input/Output Format}
% \smallskip
% \noindent\textbf{Input/Output Format \hspace{0.5em}}
% \notekw{We should motivate why this input/output make sense for learning a represetnation also add some discussion what can be learned through this procedure. We need to provide some insight why providing these data pairs in PL, NL make sense}
The input to the encoder is a noisy text sequence, while the input to the decoder is the original text with one position offset. 
% A language id symbol (e.g., <java>, <python>) is pre-pended to the decoder input to predict the sequence.
A language id symbol (e.g., <java>, <python>) is appended and prepended to the encoder and decoder inputs, respectively.
We provide a few examples in Table \ref{table:pre_training}.
The input instances are truncated if they exceed a maximum sequence length of 512.


\paragraph{Learning}
% \smallskip
% \noindent\textbf{Learning \hspace{0.5em}}
PLBART is pre-trained on $N$ languages (in our case, $N$=3), where each language $N_i$ has a collection of unlabeled instances $\mathcal{D}_i = \{x_1, \ldots, x_{n_i}\}$.
Each instance is corrupted using the noise function $f$ and we train PLBART to predict the original instance $x$ from $f(x)$.
Formally, PLBART is trained to maximize $\mathcal{L}_{\theta}$:
\begin{equation*}
    \mathcal{L}_{\theta} = \sum_{i=1}^N \sum_{j=1}^{m_i} \log P (x_j | f(x_j); \theta)
\end{equation*}
where $m_i$ is the number of sampled instances in language $i$ and the likelihood $P$ is estimated following the standard sequence-to-sequence decoding.
% by PLBART, following the standard sequence-to-sequence decoding.
% \footnote{Following the standard sequence-to-sequence decoding.}
% \notekw{PLBART is doing prediction autoregressively. It's a bit unclear what do you mean by outputs the distribution P.}

\paragraph{Optimization} 
% \smallskip
% \noindent\textbf{Optimization \hspace{0.5em}}
We train PLBART on 8 Nvidia GeForce RTX 2080 Ti GPUs for 100K steps.
The effective batch size is maintained at 2048 instances.
We use Adam ($\epsilon$ = 1e-6, $\beta_2$ = 0.98) with a linear learning rate decay schedule for optimization. 
We started the training with dropout 0.1 and reduced it to 0.05 at 50K steps and 0 at 80K steps.
This is done to help the model better fit the data \cite{liu2020multilingual}.
The total training time was approximately 276 hours (11.5 days).
All experiments are done using the Fairseq library~\cite{ott-etal-2019-fairseq}.


\subsection{Fine-tuning PLBART}
We fine-tune PLBART for two broad categories of downstream applications.

\paragraph{Sequence Generation}
% \smallskip
% \noindent\textbf{Sequence Generation \hspace{0.5em}}
PLBART has an encoder-decoder architecture where the decoder is capable of generating target sequences autoregressively.
Therefore, we can directly fine-tune PLBART on sequence generation tasks, such as code summarization, generation, and translation.
Unlike denoising pre-training, the source sequence is given as input to the encoder during fine-tuning, and the decoder generates the target sequence.
The source and target sequence can be a piece of code or text sequence.
Table \ref{table:fine_tuning} shows a few examples of input and output to and for PLBART for different generation tasks.
Note that PLBART prepends a language id to the decoded sequence; it enables fine-tuning PLBART in a multilingual setting (\eg code generation in multiple languages).\footnote{We do not perform multilingual fine-tuning in this work.}
% Note that PLBART appends a list of language ids to its vocabulary such that it can generate sequences in unseen languages, languages other than Java, Python, and English.


\paragraph{Sequence Classification}
% \smallskip
% \noindent\textbf{Sequence Classification \hspace{0.5em}}
We fine-tune PLBART on sequence classification tasks following \citet{lewis-etal-2020-bart}.
The input sequence is fed into both the encoder and decoder.
For a pair of inputs, we concatenate them but insert a special token (``</s>'') between them. 
A special token is added at the end of the input sequence.
This last token's representation from the final decoder layer is fed into a linear classifier for prediction.


\paragraph{Optimization}
% \smallskip
% \noindent\textbf{Optimization \hspace{0.5em}}
We fine-tune PLBART for a maximum of 100K steps on all the downstream tasks with 2500 warm-up steps.
We set the maximum learning rate, effective batch size, and dropout rate to 3e-5, 32 and 0.1, respectively.
The final models are selected based on the validation BLEU (in generation task) or accuracy (in classification tasks). 
Fine-tuning PLBART is carried out in one Nvidia GeForce RTX 2080 Ti GPU.
% During inference for the generation tasks, we use beam-search decoding (with beam size 5 or 10).


==> [NAACL 2021] PLBART_camera_ready/latex/relwork.tex <==
\section{Related Work}
% {\color{red} @Saikat briefly draft the related works. Focus primarily on the following two topics.}

% \subsection{Pre-training for Generation}
\paragraph{Pre-training for Language Understanding and Generation}
% \noindent\textbf{Pre-training for Language Understanding and Generation \hspace{0.5em}}
Transformer~\cite{vaswani2017attention}, a sequence-to-sequence architecture that includes an encoder and decoder, has shown tremendous promise in natural language processing (NLP), computer vision, software engineering, and more.
\citet{devlin-etal-2019-bert} first proposed to pre-train a large Transformer architecture, called BERT, to learn representations of natural language using large-scale unlabeled data in a self-supervised fashion.
Later, BERT's task-independent pre-training approach is rigorously studied~\cite{devlin-etal-2019-bert, liu2019roberta, solaiman2019release, feng2020codebert, sun2019videobert, li-etal-2020-bert-vision}. 
% All such models are trained to learn representations of natural language, image or video using large-scale unlabeled data in a self-supervised fashion. 
% In MLM, random tokens from an input sequence is masked, and
% then encodes the sequence bidirectionally. 
% then BERT is optimized to predict the missing tokens independently.
While BERT-like models have shown effectiveness in learning contextualized representation, it is not very useful in generation tasks.
GPT~\cite{radford2018improving} style models improve upon BERT for generative tasks with autoregressive pre-training; however, unlike BERT, they are not bidirectional.
% While GPT-style models are effective in the generation, they are not bidirectional as BERT.
% are only trained based on one direction generation. 
% Thus such models are not capable of learning representations in bidirectional settings. 
\citet{lewis-etal-2020-bart} introduced BART, a denoising autoencoder that uses a bidirectional encoder and an auto-regressing decoder.
% to embed the input by looking at both context directions, and a auto-regressing decoder for making it suitable for generative task. 
Similar to BART, PLBART uses denoising pre-training to cope with generative tasks and learns multilingual representations of programming and natural language jointly. 
% In addition, \tool uses one unified model for different programming languages (python and java) and natural language, so that, the model can better understand the semantic representation. 

% \subsection{Deep Learning in Software Engineering}
% \paragraph{Deep Learning in Software Engineering}
\medskip
\noindent\textbf{Deep Learning in Software Engineering \hspace{0.5em}}
There is a growing interest in automating software engineering (SE) using deep learning in the last few years. 
Vast sources of code in open source repositories and forums make deep learning feasible for SE tasks.
Code Summarization~\cite{movshovitz2013natural, allamanis2016convolutional, iyer2016summarizing, alon2018codeseq, hu2018deep, harer2019tree, ahmad-etal-2020-transformer}, Bug Detection~\cite{ray2016naturalness, li2018vuldeepecker, russell2018automated, zhou2019devign, chakraborty2020deep},  Program Repair~\cite{chen2019sequencer, chakraborty2020codit, lutellier2020coconut}, Code Translation~\cite{chen2018tree, drissi2018program, xu2020tree2tree}, Clone Detection~\cite{zhang2019novel, yu2019neural, wang2020detecting}, Code completion~\cite{li2017code, hellendoorn2017fse, parvez-etal-2018-building} are some of the tasks that are addressed with deep neural solution.
% The main challenge in all these tasks is learning effective source code or program representation. 
While most of the prior approaches use task-specific representation learning, a few works \cite{alon2019code2vec, feng2020codebert, guo2020graphcodebert, lachaux2020unsupervised, clement-etal-2020-pymt5} attempted to learn transferable representations in an unsupervised fashion.
% For instance, Code2Vec~\cite{alon2019code2vec} learns representation of code tokens using AST paths.
More closely to our work, CodeBERT~\cite{feng2020codebert} is pre-trained on bimodal data to capture the semantic interaction between the input modalities (\ie program and natural languages).
% More closely to PLBART, CodeBERT~\cite{feng2020codebert} is pre-trained like BERT and thus inherits BERT-style models' inadequacy in generative tasks. 
% However, being a BERT based model, CodeBERT inherits BERT-style models' inadequacy in generative tasks. 
More recently, GraphCodeBERT~\cite{guo2020graphcodebert} improves upon CodeBERT by leveraging data flow in source code.
In contrast, PLBART is pre-trained on large-scale data using denoising autoencoding to learn the program and natural language representations that make it effective for a broad spectrum of software engineering tasks.
% In contrast to the BERT-style models, denoising autoencoding makes PLBART better suitable for downstream generative task as well as learn the contextual representation better, helping it perform better in classification tasks. 
% In contrast, PLBART uses autoregressive decoding that makes it suitable for downstream generative task.
% as well as learn the contextual representation better, helping it perform better in classification tasks. 
% However, unlike prior works, we jointly pre-train PLBART to learn program and language representations.
% In addition, PLBART uses autoregressive decoding that makes it suitable for downstream generative task.





% {\color{red} Our ACL paper may help on aggregating references for the summarization task.}



% \subsection{Code Generation}



% \subsection{Code Translation}





==> [NAACL 2021] PLBART_camera_ready/latex/setup.tex <==
\section{Experiment Setup}
\label{sec:exp_setup}

\input{table/github_datastat}

% \subsection{Evaluation Objectives}
% To understand PLBART's performance in a broader context, we evaluate PLBART on several tasks. 
% More specifically, our evaluation focus is on -- ({\tt i}) understanding of program syntax, ({\tt ii}) understanding of program semantics, ({\tt iii}) correct synthesis of program, ({\tt iv}) understading the interaction between PL and NL.
% Such an exhaustive evaluation helps us establishing PLBART's usefulness in a wide variety of PLUG tasks. 

To understand PLBART's performance in a broader context, we evaluate PLBART on several tasks. 
Our evaluation focuses on assessing PLBART's ability to capture rich semantics in source code and associated natural language text.
% Such an exhaustive evaluation helps us establishing PLBART's usefulness in a wide variety of PLUG tasks. 

\subsection{Evaluation Tasks}
% To understand PLBART's performance in a broader context, we evaluate PLBART on several tasks. Such an exhaustive evaluation helps us establishing PLBART's usefulness in a wide variety of program understanding and generation tasks. 
We divide the evaluation tasks into four categories.
The evaluation task datasets are summarized in Table \ref{tab:dataset_task}.
We use CodeXGLUE~\cite{CodeXGLUE} provided public dataset and corresponding train-validation-test splits for all the tasks. 


% \smallskip
% \noindent\textbf{Code Summarization \hspace{0.5em}}
\paragraph{Code Summarization}
refers to the task of generating a natural language (English) summary from a piece of code. We fine-tune PLBART on summarizing source code written in six different programming languages, namely, Ruby, Javascript, Go, Python, Java, and PHP.
% We use the CodeSearchNet~\cite{husain2019codesearchnet} in this task.

% \smallskip
% \noindent\textbf{Code Generation \hspace{0.5em}}
\paragraph{Code Generation} 
is exactly the opposite of code summarization. It refers to the task of generating a code (in a target PL) from its NL description.
% Given an NL description of a code, the goal in this task is to generate the code in a target PL.
We fine-tune PLBART on the Concode dataset~\cite{iyer-etal-2018-mapping}, where the input is a text describing class member functions in Java and class environment, the output is the target function.
% Note that, in code summarization and generation, PLBART deals with both PL and NL, thus these two tasks evaluate PLBART's understanding of PL and NL.

% \smallskip
% \noindent\textbf{Code Translation \hspace{0.5em}} 
\paragraph{Code Translation}
requires a model to generate an equivalent code in the target PL from the input code written in the source PL.
Note that the source and target PL can be the same.
Hence, we consider two types of tasks in this category.

The first task is a typical PL translation task, translating a code \ie from Java code to C\#, and vice versa.
In this task, the semantic meaning of the translated code should exactly match the input code. 
Thus, this task evaluates PLBART's understanding of program semantics and syntax across PL.
% We evaluate PLBART on translating source code between Java and C\# using the translation dataset from CodeXGLUE~\cite{CodeXGLUE}.
The second task we consider is program repair. 
% In this task, the input and output are in the same language (\ie Java), but there are semantic differences between the input and the output. 
In this task, the input is a buggy code, and the output is a modified version of the same code which fixes the bug. 
% More precisely, the input is a buggy code, and the output is a modified version of the same code which fixes the bug. 
% We evaluate PLBART on two different datasets (Java$_{small}$, Java$_{medium}$) proposed by \citet{tufano2019empirical}. 
This task helps us understand PLBART's ability to understand code semantics and apply semantic changes in the code. 

% \smallskip
% \noindent\textbf{Code Classification \hspace{0.5em}}
\paragraph{Code Classification}
% To further asses PLBART's ability in program understanding, 
aims at predicting the target label given a single or a pair of source code. 
We evaluate PLBART on two classification tasks. 
The first task is clone detection, where given a pair of code, the goal is to determine whether they are clone of each other (similar to paraphrasing in NLP).
% We use the clone detection dataset from \citet{wang2020detecting} that contains pair of java code and corresponding clone annotation. 
The second task is detecting whether a piece of code is vulnerable.
% We use~\citet{zhou2019devign}'s proposed dataset for evaluation on this task. 
% Note that, this task has limited annotations and thus 
This task help us gauging PLBART's effectiveness in program understanding in an unseen PL since the code examples in this task are written in C/C++.





\subsection{Evaluation Metrics}

% \noindent\textbf{BLEU \hspace{0.5em}} 
\paragraph{BLEU} 
computes the n-gram overlap between a generated sequence and a collection of references.
% evaluates the similarity between a generated sequence and a collection of references by measuring the n-gram overlap.
We use corpus level BLEU~\cite{papineni-etal-2002-bleu} score for all the generation tasks, except code summarization where we use smoothed BLEU-4 score \cite{lin-och-2004-orange} following \citet{feng2020codebert}. 
% For all code generation tasks, we use corpus level BLEU~\cite{} score. 
% is the BLEU-4 score ~\notewa{Please confirm this.}

% {\color{blue} No, for code summarization, we use smoothed BLEU-4 score, otherwise in all places we use BLEU score which is the geometric mean of BLEU-1-4.}

% \smallskip
% \noindent\textbf{{CodeBLEU} \hspace{0.5em}} 
\paragraph{CodeBLEU}
is a metric for measuring the quality of the synthesized code~\cite{ren2020codebleu}. 
Unlike BLEU, CodeBLEU also considers grammatical and logical correctness based on the abstract syntax tree and the data-flow structure. 
% Unlike BLEU, CodeBLEU also accounts for the syntactic similarity (with AST), and semantic similarity (with data flow).
% A generated code may have large similarity with the reference, and thus results in high BLEU score. 
% However, the generated code may not syntactically/semantically valid/similar to the reference, and CodeBLEU will indicate that with a lower score. 
% On the other hand, BLEU score between a generated code and reference having completely different set of variables or function names will be low. 
% In contrast, higher CodeBLEU will indicate their syntactic and data flow similarity.
% Consider a generated code and reference having completely different set of variables or function names, but the code is syntactically/semantically valid/similar to the reference.
% Although, the resulting BLEU score will be low, but CodeBLUE score will be high.

% \smallskip
% \noindent\textbf{{Exact Match (EM)} \hspace{0.5em}} 
\paragraph{Exact Match (EM)}
evaluates if a generated sequence exactly matches the reference. 
% EM is a very stringent metric and signifies the lower bound of performance for any generative task.
% For code generation tasks, specifically in program repair, exact match accuracy is crucial, since unless a model can generate the exact reference, the output will not be considered completely bug-free. 


% {\color{red} @Saikat although simple, but we should define accuracy as it is used in translation and program repair task. We can mention this metric with exact match, but need to ensure readers do not confuse them. -- Changed to EM in Code Translation and Program Repair}





\subsection{Baseline Methods}
We compare PLBART with several state-of-the-art models and broadly divide them into two categories.
First, the models that are trained on the evaluation tasks from scratch, and second, the models that are pre-trained on unlabeled corpora and then fine-tuned on the evaluation tasks.

% \vspace{1mm}
% \noindent
% \textbf{Fine Tuned Models}
\subsubsection{Training from Scratch}

% We train the following two models from scratch.

% \smallskip
\noindent{\textbf{Seq2Seq}~\cite{luong-etal-2015-effective}\hspace{0.5em}} 
% \paragraph{Seq2Seq} 
% is an LSTM based sequence-to-sequence model with attention mechanism \cite{luong-etal-2015-effective}. 
% Vocabulary is constructed a using byte-pair encoding \cite{feng2020codebert}. 
% No copying mechanism is adopted in this model.
is an LSTM based Seq2Seq model with attention mechanism. Vocabulary is constructed using byte-pair encoding.
% \cite{feng2020codebert}. 

\medskip
\noindent{\textbf{Transformer}~\cite{vaswani2017attention}\hspace{0.5em}}
% \paragraph{Transformer} 
is the base architecture of PLBART and other pre-trained models.
% A randomly initialized 6 layers Transformer is fine-tuned on the evaluation tasks. 
Transformer baseline has the same number of parameters as PLBART.
Hence, a comparison with this baseline demonstrates the direct usefulness of pre-training PLBART. 


% \noindent\textbf{Pretraining methods}
\subsubsection{Pre-trained Models}
As described in section~\ref{sec:method}, PLBART consists of an encoder and autoregressive decoder. 
% We evaluate on other pre-trained model categories. Our first baseline pre-trained model category is BERT style models where only the encoder is pretrained. Our second baseline model category is GPT style models with only autoregressive pre-trained decoder.
We compare PLBART on two categories of pre-trained models. First, the encoder-only models (\eg RoBERTa, CodeBERT, and GraphCodeBERT) that are combined with a randomly initialized decoder for task-specific fine-tuning. The second category of baselines include decoder-only models (CodeGPT) that can perform generation autoregressively.


\input{table/code_to_text}



% \notekw{I think you should empahsize here again what is the key different between your and these appraoches to somehow motivate why you choose these baseline. }
\medskip
\noindent\textbf{RoBERTa, RoBERTa (code) \hspace{0.5em}} 
% \paragraph{RoBERTa, RoBERTa (code)}
are RoBERTa \cite{liu2019roberta} model variants.
While RoBERTa is pre-trained on natural language, RoBERTa (code) is pre-trained on source code from CodeSearchNet~\cite{husain2019codesearchnet}.
% (see \Cref{tab:dataset_task} for details).
% CodeSearchNet consists of 6.4M functions written in 6 programming languages as noted in Table \ref{tab:dataset_task} (task: summarization).

\medskip
\noindent{\textbf{CodeBERT}~\cite{feng2020codebert} \hspace{0.5em}} 
% \paragraph{CodeBERT} \cite{feng2020codebert}
combines masked language modeling (MLM)~\cite{devlin-etal-2019-bert} with replaced token detection objective~\cite{clark2020electra} to pretrain a Transformer encoder.
% CodeBERT is pre-trained on 2.4M code-text pairs from CodeSearchNet.
% To perform generation tasks, CodeBERT is combined with a randomly initialized autoregressive decoder.

\medskip
\noindent{\textbf{GraphCodeBERT} \cite{guo2020graphcodebert} \hspace{0.5em}}
% \paragraph{GraphCodeBERT}  
is a concurrent work with this research which improved CodeBERT by modeling the data flow edges between code tokens.
% In addition to MLM, they used structure-aware pre-training objectives.
We report GraphCodeBERT's performance directly from the paper since their implementation is not publicly available yet.



\medskip
\noindent\textbf{GPT-2, CodeGPT-2, and CodeGPT-adapted \hspace{0.5em}}
% \paragraph{GPT-2, CodeGPT-2, and CodeGPT-adapted}
are GPT-style models.
While GPT-2 \cite{radford2019language} is pretrained on NL corpora, CodeGPT-2 and CodeGPT-adapted are pretrained on CodeSearchNet \cite{CodeXGLUE}.
Note that, CodeGPT-adapted starts from the GPT-2 checkpoint for pre-training.

% For GPT-2, We use OpenAI GPT-2 model and fine-tune on Concode dataset. When training, we concatenate NL description and source code as an example, training as a language model (calculating loss of source code only). CodeGPT and CodeGPT-adapted are pre-trained models on code. You could refer here (https://git.io/JkkAW) for details.

% \smallskip
% \noindent All pre-trained models are loaded in Sequence to Sequence transformer and fine-tuned for the appropriate dataset for the generative tasks. For the classification task, however, we add a feed-forward classification layer after the last token in the decoder. To compare in a fair ground, we use the same hyperparameter settings for \tool and all the baselines. 




==> [NAACL 2021] PLBART_camera_ready/table/code_to_code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
% \resizebox{\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c c c| c c c}
\hline
\multirow{ 2}{*}{Methods} & \multicolumn{3}{c|}{Java to C\#} & \multicolumn{3}{c}{C\# to Java} \\ 
\cline{2-7}
& BLEU & EM & CodeBLEU & BLEU & EM & CodeBLEU \\ 
\hline
Naive Copy & 18.54 & 0 & 34.20 & 18.69 & 0 & 43.04 \\
PBSMT & 43.53 & 12.50 & 42.71 & 40.06 & 16.10 & 43.48 \\
Transformer & 55.84	& 33.00	& 63.74	& 50.47	& 37.90	& 61.59 \\
RoBERTa (code)  & 77.46 & 56.10 & 83.07 & 71.99 & 57.90 & 80.18 \\
CodeBERT & 79.92 & 59.00 & 85.10 & 72.14 & 58.80 & 79.41 \\ 
GraphCodeBERT & 80.58 & 59.40 & - & 72.64 & 58.80 & - \\\hline

\tool  & {\bf 83.02} & {\bf 64.60} & {\bf 87.92} & {\bf 78.35} & {\bf 65.00} & {\bf 85.27} \\
\hline
\end{tabular}
% }
\caption{
Results on source code translation using Java and C\# language dataset introduced in \cite{CodeXGLUE}.
PBSMT refers to phrase-based statistical machine translation where the default settings of Moses decoder \cite{koehn-etal-2007-moses} is used. The training data is tokenized using the RoBERTa \cite{liu2019roberta} tokenizer. 
% We report GraphCodeBERT's performance from the paper~\cite{guo2020graphcodebert}.
}
% }
\label{table:code_translation}
% \vspace{-2mm}
\end{table*}



==> [NAACL 2021] PLBART_camera_ready/table/code_to_text.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
\centering
% \resizebox{\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c c c c c c|c}
\hline
Methods & Ruby & Javascript & Go & Python & Java & PHP & Overall \\
\hline
Seq2Seq &  9.64	& 10.21	& 13.98	& 15.93	& 15.09	& 21.08	& 14.32 \\
Transformer & 11.18	& 11.59	& 16.38	& 15.81	& 16.26	& 22.12 & 15.56 \\
RoBERTa  & 11.17 & 11.90 & 17.72 & 18.14 & 16.47 & 24.02 & 16.57 \\
CodeBERT & 12.16 & 14.90 & 18.07 & 19.06 & 17.65 & {\bf 25.16} & 17.83 \\ \hline
\tool & {\bf 14.11} & {\bf 15.56} & {\bf 18.91} & {\bf 19.30} & {\bf 18.45} & 23.58 & {\bf 18.32} \\
\hline
\end{tabular}
% }
\caption{Results on source code summarization, evaluated with smoothed BLEU-4 score. The baseline results are reported from \citet{feng2020codebert}.}
% }
\label{table:code_to_text}
% \vspace{-2mm}
\end{table*}


==> [NAACL 2021] PLBART_camera_ready/table/github_datastat.tex <==
\begin{table*}[!ht]
\centering
% \small
\begin{tabular}{l|l|l|r|r|r}
\hline
Task & {Dataset} & Language & Train & Valid & Test \\
\hline
\multirow{6}{*}{Summarizaion} & \multirow{6}{*}{\citet{husain2019codesearchnet}} &Ruby & 24,927& 1,400& 1,261\\
& & Javascript & 58,025	& 3,885 &	3,291 \\
& & Go & 167,288	&   7,325	&   8,122\\
& & Python & 251,820	&   13,914	&   14,918 \\
& & Java & 164,923	&   5,183	&   10,955 \\
& & PHP & 241,241	&   12,982	&   14,014\\
\hline
Generation  & \citet{iyer-etal-2018-mapping} & NL to Java & 100,000 & 2,000 & 2,000\\
\hline
\multirow{4}{*}{Translation} & \multirow{2}{*}{Code-Code \cite{CodeXGLUE}}  & Java to C\# & 10,300 & 500 & 1,000\\
& & C\# to Java & 10,300 & 500 & 1,000\\
\cline{2-6}
& Program Repair & Java$_{small}$ & 46,680 & 5,835 & 5,835\\
& \cite{tufano2019empirical}& Java$_{medium}$ & 52,364 & 6,545 &6,545\\
\hline
\multirow{4}{*}{Classification}& Vulnerability Detection & \multirow{2}{*}{C/C++} & \multirow{2}{*}{21,854} & \multirow{2}{*}{2,732} & \multirow{2}{*}{2,732} \\
& \cite{zhou2019devign} & & & & \\
\cline{2-6}
& Clone Detection & \multirow{2}{*}{Java} & \multirow{2}{*}{100,000} & \multirow{2}{*}{10,000} & \multirow{2}{*}{415,416} \\
& \cite{wang2020detecting} & & & & \\
\hline
\end{tabular}
\caption{Statistics of the downstream benchmark datasets.}
\label{tab:dataset_task}
% \vspace{-2mm}
\end{table*}

==> [NAACL 2021] PLBART_camera_ready/table/pretrain_data.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\small
\begin{tabular}{@{\hskip 0.05in}l@{\hskip 0.05in} r@{\hskip 0.1in} r@{\hskip 0.1in} r@{\hskip 0.05in}}
\hline
 & Java & Python & NL \\ 
\hline
All Size & 352 GB & 224 GB & 79 GB \\
All - Nb of tokens & 36.4 B & 28 B & 6.7 B \\
All - Nb of documents & 470 M & 210 M & 47 M \\
\hline
\end{tabular}
}
\caption{
Statistics of the data used to pre-train PLBART. ``Nb of documents'' refers to the number of functions in Java and Python collected from Github and the number of posts (questions and answers) in the natural language (English) from StackOverflow.
}
\label{table:pretrain_data}
% \vspace{-2mm}
\end{table}


==> [NAACL 2021] PLBART_camera_ready/table/repair.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[!ht]
% \centering
% \resizebox{\linewidth}{!}{%
% % \small
% % \def\arraystretch{1.1}%
% \begin{tabular}{l|c c c| c c c}
% \hline
% \multirow{ 2}{*}{Methods} & \multicolumn{3}{c|}{Small} & \multicolumn{3}{c}{Medium} \\ 
% \cline{2-7}
% & BLEU & Accuracy & CodeBLEU & BLEU & Accuracy & CodeBLEU \\ 
% \hline
% Naive Copy & {\bf 78.06} & 0 & 81.39 & 90.91 & 0 & 88.54 \\
% Seq2Seq & 76.76	& 10.00 & - & 72.08 & 2.50	& - \\
% Transformer \cite{vaswani2017attention} & 77.21	& 14.70 & 73.31 & 89.25 & 3.70 & 81.72 \\
% CodeBERT \cite{feng2020codebert} & 77.42 & 16.40 & {\bf 75.58} & {\bf 91.07} & 5.16 & {\bf 87.52} \\
% CodeBART (this work) & 77.02 & {\bf 19.21} & 75.18 & 88.50 & {\bf 8.98} & 85.27 \\
% \hline
% \end{tabular}
% }
% \caption{caption.}
% % }
% \label{table:bug_fix}
% % \vspace{-2mm}
% \end{table*}

% \begin{table}[!ht]
% \centering
% \resizebox{\linewidth}{!}{%
% % \small
% % \def\arraystretch{1.1}%
% \begin{tabular}{l|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Small} & \multicolumn{2}{c}{Medium} \\ 
% \cline{2-5}
% & Acc. & CodeBL. & Acc. & CodeBL. \\ 
% \hline
% Naive Copy & 0 & {\bf 81.39} & 0 & {\bf 88.54} \\
% Seq2Seq & 10.00 & - & 2.50	& - \\
% Transformer  & 14.70 & 73.31 & 3.70 & 81.72 \\
% CodeBERT & 16.40 & 75.58 & 5.16 & 87.52 \\
% GraphCodeBERT & 17.30 & - & {\bf 9.10} & - \\
% \hline
% \tool & {\bf 19.21} & 75.18 & {\bf 8.98} & 85.27 \\
% \hline
% \end{tabular}
% }
% \caption{Results on program repair (in Java).}
% % }
% \label{table:bug_fix}
% % \vspace{-2mm}
% \end{table}


\begin{table}[!ht]
\centering
\resizebox{\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c@{\hskip 0.1in} c|c@{\hskip 0.1in} c}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Small} & \multicolumn{2}{c}{Medium} \\ 
\cline{2-5}
& EM & BLEU & EM & BLEU \\ 
\hline
Naive Copy & 0 & {78.06} & 0 & {90.91} \\
Seq2Seq & 10.00 & 76.76 & 2.50	& 72.08 \\
Transformer  & 14.70 & 77.21 & 3.70 & 89.25 \\
CodeBERT & 16.40 & 77.42 & 5.16 & \textbf{91.07} \\
GraphCodeBERT & 17.30 & \textbf{80.58} & {\bf 9.10} & 72.64 \\
\hline
\tool & {\bf 19.21} & 77.02 & {8.98} & 88.50 \\
\hline
\end{tabular}
}
\caption{Results on program repair (in Java).}
% }
\label{table:bug_fix}
% \vspace{-1mm}
\end{table}



==> [NAACL 2021] PLBART_camera_ready/table/text_to_code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c c c}
\hline
Methods & EM & BLEU & CodeBLEU \\ 
\hline
Seq2Seq & 3.05 & 21.31 & 26.39 \\
\citet{guo-etal-2019-coupling} & 10.05 & 24.40 & 29.46 \\
\citet{iyer-etal-2019-learning} & 12.20 & 26.60 & - \\
GPT-2 & 17.35 & 25.37 & 29.69 \\
CodeGPT-2 & 18.25 & 28.69 & 32.71 \\
CodeGPT-adapted & {\bf 20.10} & 32.79 & 35.98 \\ \hline
PLBART & 18.75 & {\bf 36.69} & {\bf 38.52} \\
\hline
\hline
PLBART$_{10K}$ & 17.25 & 31.40 & 33.32 \\
PLBART$_{20K}$ & 18.45 & 34.00 & 35.75 \\
% \tool$_{30K}$ & 18.65 & 34.84 & 37.08 \\
PLBART$_{50K}$ & 17.70 & 35.02 & 37.11 \\
% CodeBART$_{80K}$ & 18.45 & 36.76 & 39.01 \\
\hline
\end{tabular}
}
\caption{Results on text-to-code generation task using the CONCODE dataset \cite{iyer-etal-2018-mapping}.}
% }
\label{table:concode}
% \vspace{-2mm}
\end{table}

==> [NAACL 2021] PLBART_camera_ready/table/vulnerability.tex <==
\begin{table}[t]
\centering
% \resizebox{\linewidth}{!}{%
% \small
% \def\arraystretch{1.1}%
\begin{tabular}{l|c c}
\hline
\multirow{2}{*}{Tasks} & Vulnerability & Clone \\ 
& Detection & Detection \\
\hline
Transformer & 61.64  & - \\
CodeBERT & 62.08 & 96.5 \\
GraphCodeBERT & - & 97.1 \\ 
\hline
\tool & {\bf 63.18} & {\bf 97.2} \\
\hline
\end{tabular}
% }
\caption{Results on the vulnerable code detection (accuracy) and clone detection (F1 score) tasks.}
% }
\label{table:classification}
% \vspace{-3mm}
\end{table}

==> images/qual_example_concode_2.tex <==
\begin{figure}[t]
% \centering
\rule{\linewidth}{0.6pt}\vspace{-1mm}
{{\bf Input text:} returns the count to which the specified key is mapped in this frequency counter , or 0 if the map contains no mapping for this key .}
\\ [6pt]
\begin{subfigure}{0.50\textwidth}
\caption{\underline{Reference Code}}
\vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
Integer function (T arg0) { 
	Integer loc0 = counter.get(arg0); 
	if (loc0 == null) { 
		return 0 ;
	} 
	return loc0; 
}
\end{lstlisting}
\end{tabular}
\label{tab:ref_code_concode}
\end{subfigure}%
\\ \\
% \vspace{2mm}
\begin{subfigure}{0.50\textwidth}
\lstset{escapechar=@,style=CustomJava}
\caption{\underline{Generated Code}}
\vspace{-3mm}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
int function (T arg0) { 
	Integer loc0 = counter.get(arg0); 
	if (loc0 == null) { 
		return 0 ;
	} 
	else { 
		return loc0;
	} 
}
\end{lstlisting}
\end{tabular}
% \vspace{1mm}
\label{tab:gen_code_concode}
\end{subfigure}
% \vspace{1mm}
\rule{\linewidth}{0.6pt}
\caption{
An example of generated code by PLBART that is syntactically and semantically valid, but does not match the reference.
}
\label{concode_example}
% \vspace{-2mm}
\end{figure}
